Exploring the Meaningfulness of Nearest Neighbor Search in High-Dimensional Space

Dense high dimensional vectors are becoming increasingly vital in fields such as computer vision, machine learning, and large language models (LLMs), serving as standard representations for multimodal data. Now the dimensionality of these vector can exceed several thousands easily. Despite the nearest neighbor search (NNS) over these dense high dimensional vectors have been widely used for retrieval augmented generation (RAG) and many other applications, the effectiveness of NNS in such a high-dimensional space remains uncertain, given the possible challenge caused by the "curse of dimensionality." To address above question, in this paper, we conduct extensive NNS studies with different distance functions, such as $L_1$ distance, $L_2$ distance and angular-distance, across diverse embedding datasets, of varied types, dimensionality and modality. Our aim is to investigate factors influencing the meaningfulness of NNS. Our experiments reveal that high-dimensional text embeddings exhibit increased resilience as dimensionality rises to higher levels when compared to random vectors. This resilience suggests that text embeddings are less affected to the "curse of dimensionality," resulting in more meaningful NNS outcomes for practical use. Additionally, the choice of distance function has minimal impact on the relevance of NNS. Our study shows the effectiveness of the embedding-based data representation method and can offer opportunity for further optimization of dense vector-related applications.

==> tables/models.tex <==
\begin{table}[!ht]
    \centering
    \small
    \begin{threeparttable}
        \begin{tabular}{|l|c|c|c|c|}
            \toprule
            \textbf{Model Name} & \textbf{Param} & \textbf{Max Input} & \textbf{Dim} & \textbf{Architecture} \\
            \midrule
            all-MiniLM-L6-V2 \cite{miniLM} & 22.7M & 256 & 384 & Encoder \\
            bert-base-nli-mean-tokens \cite{sentence-bert} & 109M & 512 & 768 & Encoder \\
            Alibaba-NLP/gte-large-en-v1.5 \cite{gte-large} & 434M & 8192 & 1024 & Encoder \\
            Wissam42/sentence-croissant-llm-base \cite{croissantllm} & 1280M & 2048 & 2048 & Decoder \\
            Alibaba-NLP/gte-Qwen2-7B-instruct \cite{gte-qwen} & 7.61B & 131072 & 3584 & Decoder \\
            nvidia/NV-Embed-v1 \cite{nvembed} & 7.85B & 32768 & 4096 & Decoder \\
            \bottomrule
        \end{tabular}
    \end{threeparttable}
    \caption{Comparison of different models.}
    \label{tab:text_model2}
\end{table}


==> tex_files/introduction.tex <==
High dimensional vector is a crucial component of the research in many fields, like Computer Vision(CV), Machine Learning(ML), as well as Database. In Computer Vision, with the Convolution Neural Network (CNN) \cite{resnet}\cite{vgg}\cite{squeezenet}, high-dimensional vector enables the representation of images in a unified and structured format, where each dimension of the vector represents features like shape, color, texture, and spatial relations. Nowadays, Large Language Model is definitely the center of various research. During the training and inference of LLMs, different types of unstructured data, like text, image, are tokenized into high-dimensional embeddings as the input data for LLMs. Despite LLM exhibits fabulous ability in many areas, hallucination \cite{hallucination1}\cite{hallucination2} is still one of the most concerning issue in the community. To tackle this problem, Retrieval Augmentation Generation (RAG) is considered as the most suitable choice. In RAG system, massive amount of data is stored in the knowledge base (vector database\cite{milvus}) as high-dimensional embeddings, providing and efficient and meaningful approach to store huge unstructured data. In short, high-dimensional vector is of great importance in many senses, which enables the interaction between physical world and machine intelligence.

What's more, Nearest Neighbor Search (NNS) has been a popular topic in the database and machine learning for decades, whose algorithm serves as the key component of the LLM-RAG system. The goal is to retrieve the most distance close vector in the dataset. As the cardinality and dimensionality of dataset increase, traditional approach, which searches for the exact result, is incapable of solving the problem efficiently, Approximate Nearest Neighbor Search (ANNS) became the focus of the research of NN search. In Approximate Nearest Neighbor Search, algorithms are commonly divided into four categories, including tree based \cite{kd-tree}\cite{ball-tree}\cite{cover-tree}, hashing based\cite{pm-lsh}\cite{QALSH}, quantization based\cite{pq-paper}\cite{opq-paper}, and graph based\cite{hnsw}. Research has been done for each categories of algorithm during the past few decades and numerous algorithms are proposed to tackle various problems of distinct settings.

Although algorithms for ANN search has been well studied, as the dimensionality of the dataset increases to a completely new level, especially for text embeddings, ANN algorithms might start to suffer from a classical problem: \textit{The Curse of Dimensionality} \cite{cod}, which was initially proposed by Richard E. Bellman, referring to various phenomena that occurs in analyzing high-dimensional vector. Specifically, in NN Search, as the dimensionality increases, the volume of vector space grows exponentially, resulting in a sparse distribution of vectors. In a more extreme case, all data points are evenly distributed in the space or on the surface of a sphere, giving rise to little discrimination among different data points, in terms of distance. As a consequence, the property of proximity is significantly undermined and the distance between any arbitrary two vectors converges, indicating that the distance metric is incapable of distinguish different neighbors. and the NN search will become less meaningful.

Naturally, a question rises regarding the impact of dimensionality on the meaningfulness of nearest neighbor (NN) search. Specifically, how significantly does increasing the dimensionality influence the meaningfulness of NN search, especially in high-dimensional spaces? If the meaningfulness of high-dimensional vectors degrades substantially with an increasing dimensionality, it turns into question the efficacy of NN search in such spaces. Conversely, is it possible that certain types of high-dimensional vectors are inherently more resilient to the adverse effects of dimensionality, thus preserving the meaningfulness of NN search, without being impacted by the curse of dimensionality?

Apart from dimensionality, which is one of the most important property of the vector, we might rise the doubt, what other factors of the high-dimensional data might impact the meaningfulness of nearest neighbor search problem ?

To resolve questions and concerns aforementioned, we conduct this study on high-dimensional vector in context of the nearest neighbor search, aiming to provide some insight on various types of vector in the high-dimensional space. To better fit the real-world situation, not only we used some existing prestigious datasets, also we use several performant and prestigious embedding model, to generate the high-dimensional embeddings for text and image data of the real world. Apart from the dataset, the quantitative measure is also an important component of entire of the study. Specifically, we use the concept of Relative Contrast, which measures the meaningfulness of the dataset in nearest neighbor search and it will be discussed in detail in the coming sections. 

Specifically, the paper is organized as the following. Firstly, it starts by investigating if the distance function would impact the result and meaningfulness of the NN search, where we include three popular distance functions: Manhattan, Euclidean, as well as the Angular distance and various types of vector are taken into consideration simultaneously (random, image feature vector, image embedding, and text embedding). Then, we turn to the most important component of the entire study: Dimensionality. Specifically, we studied how the dimensionality would impact the meaningfulness of vectors, where the random vector and text embeddings are involved in the experiment and discussion.

In addition, in the appendix section, we provide an extensive study on how different generation method of high-dimensional embedding, of the text and image data, would impact the meaningfulness of the NN search. Also, we provide an overview on the impact of the embedding models on the text dataset. 

==> tex_files/nns_metrics.tex <==
\label{lid_rc}
In this section, we discuss in detail the reason why RC is selected as the only measure for the meaningfulness of the nearest neighbor search.

Firstly, despite both RC\cite{rc-paper} and LID\cite{lid-paper,lid-estimate} generate the similar measure of the meaningfulness of the nearest neighbor search, scopes are still different. And this difference could be partially derived from the definition to RC and LID. Specifically, Relative Contrast puts more emphasis on describing the separation of distances between the mean and the nearest neighbors, providing an insight regarding the distinctiveness of the data points in NN search, as well as the meaningfulness of the nearest neighbor. On the contrary, LID focuses on the intrinsic dimensionality of the data around the query point, which is used to describe the local complexity or difficulty of the dataset. Thus, from the perspective of the original definition of RC and LID, RC is the most suitable one to measure the idea of meaningfulness. 

Then, we conduct an experiment, using $25$ various vector dataset,  to evaluate the homogeneity of two different metrics. In Fig.\ref{fig:rc-lid}, it shows that the RC and LID exhibit almost identical behaviour. Simply speaking, if a dataset is considered to be simple by one metric, the other metric will give the same comment, vice versa. Please note that, as the RC behaves in a completely opposite manner, where a higher RC indicates more a meaningful dataset while a higher LID indicates a less meaningful dataset, we take the negative of RC. What's more, as the scale of RC and LID is different, to ensure the readability of the graph, Min-Max normalization is applied to both RC and LID. 

\begin{figure}[htp]
    \centering
    \includegraphics[width=\textwidth]{graph/rc-lid.pdf}
    \caption{Compare the homogeneity of RC and LID}
    \label{fig:rc-lid}
\end{figure}

Considering the nature of RC and LID, as well as the experiment result in Figure: \ref{fig:rc-lid}, Relative Contrast is considered as the only measure for the meaningfulness of NN search in this study. 


==> tex_files/results.tex <==
\section{Evalution and Analysis}

In this section, we we will present the experimental result of previous section three major factors (generation method, distance function, and dimensionality), and conduct some brief analysis on the results. 

\input{tex_files/impact_dist.tex}
